Data splitting improves statistical performance in overparametrized regimes

While large training datasets generally offer improvement in model performance, the training process becomes computationally expensive and time consuming. Distributed learning is a common strategy to reduce the overall training time by exploiting multiple computing devices. Recently, it has been observed in the single machine setting that overparametrization is essential for benign overfitting in ridgeless regression in Hilbert spaces. We show that in this regime, data splitting has a regularizing effect, hence improving statistical performance and computational complexity at the same time. We further provide a unified framework that allows to analyze both the finite and infinite dimensional setting. We numerically demonstrate the effect of different model parameters.

==> macros_nicole.tex <==


\RequirePackage{wasysym }
%\RequirePackage[isolatin]{inputenc}
\RequirePackage{comment}
\RequirePackage{graphicx}
\RequirePackage{amsmath}%,amsfonts}
\RequirePackage{color}
\usepackage{bbold}
\usepackage{colortbl}
\usepackage{xcolor}


\definecolor{blue}{rgb}{0.6, 0.4, 1.0} %{0.0,0.0,0.55}
%\definecolor{blue}{rgb}{0.0,0.0,0.55}
\definecolor{red}{rgb}{0.75,0.0,0.0}
\definecolor{green}{rgb}{0.0,0.5,0.0}
\definecolor{bluebell}{rgb}{0.64, 0.64, 0.82}
\definecolor{amethyst}{rgb}{0.6, 0.4, 0.8}
\definecolor{applegreen}{rgb}{0.55, 0.71, 0.0}
\definecolor{awesome}{rgb}{1.0, 0.13, 0.32}
\definecolor{caribbeangreen}{rgb}{0.0, 0.8, 0.6}
 	
\newcommand{\blue}{\color{blue}}
\newcommand{\green}{\color{green}}
\newcommand{\red}{\color{red}}
 
\newcommand{\magenta}{\color{magenta}}
\newcommand{\notice}[1]{\color{magenta} #1}


%\ifx \skiptheorems \thiscommandisnotdefinedtralala  
                 

\RequirePackage{amsthm}


\newtheorem{theorem}{Theorem}[section]
\newtheorem{definition}[theorem]{Definition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}

\newtheorem{assumption}[theorem]{Assumption}
% 
% \theoremstyle{remark}
\newtheorem{question}[theorem]{Question}
\newtheorem{example}[theorem]{Example}
\newtheorem{remark}[theorem]{Remark}



%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{assumption}[theorem]{Assumption}


%\theoremstyle{definition}
%\newtheorem{definition}[theorem]{Definition}
%\newtheorem{property}[theorem]{Property}
%\newtheorem{example}[theorem]{Example}

%\theoremstyle{remark}
%\newtheorem{remark}[theorem]{Remark}


\newcommand{\bias}{\widehat{{\rm Bias}}}
\newcommand{\var}{\widehat{{\rm Var}}}
\newcommand{\SNR}{{\rm SNR}}


\DeclareMathOperator{\supp}{supp}

\newcommand{\no}{\nonumber}

\newcommand{\eins}{\mathbb{1} }
% Fonts

\newcommand{\mtc}{\mathcal}
\newcommand{\mbf}{\mathbf}

% Some black magic to remove annoying extra spaces before/after \left* and \right*

\let\originalleft\left
\let\originalright\right
\renewcommand{\left}{\mathopen{}\mathclose\bgroup\originalleft}
\renewcommand{\right}{\aftergroup\egroup\originalright}


% Accents tildes over/underline etc

\newcommand{\wt}[1]{{\widetilde{#1}}}
\newcommand{\wh}[1]{{\widehat{#1}}}
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\ul}[1]{\underline{#1}}



\RequirePackage{xstring}

\newcommand{\ind}[1]{{\mbf{1}\{#1\}}}
\newcommand{\paren}[2][a]{%
\IfEqCase{#1}{%
{a}{\left(#2\right)}%
{0}{(#2)}%
{1}{\big(#2\big)}%
{2}{\Big(#2\Big)}%
{3}{\bigg(#2\bigg)}%
{4}{\Bigg(#2\Bigg)}%
}[\PackageError{paren}{Undefined option to paren: #1}{}]%
}
\newcommand{\norms}[2][a]{%
\IfEqCase{#1}{%
{a}{\left\lVert#2\right\rVert}%
{0}{\lVert#2\rVert}%
{1}{\big\lVert#2\big\rVert}%
{2}{\Big\lVert#2\Big\rVert}%
{3}{\bigg\lVert#2\bigg\rVert}%
{4}{\Bigg\lVert#2\Bigg\rVert}%
}[\PackageError{norm}{Undefined option to norm: #1}{}]%
}
\newcommand{\brac}[2][a]{%
\IfEqCase{#1}{%
{a}{\left[#2\right]}%
{0}{[#2]}%
{1}{\big[#2\big]}%
{2}{\Big[#2\Big]}%
{3}{\bigg[#2\bigg]}%
{4}{\Bigg[#2\Bigg]}%
}[\PackageError{brac}{Undefined option to brac: #1}{}]%
}
\newcommand{\inner}[2][a]{%
\IfEqCase{#1}{%
{a}{\left\langle#2\right\rangle}%
{0}{\langle#2\rangle}%
{1}{\big\langle#2\big\rangle}%
{2}{\Big\langle#2\Big\rangle}%
{3}{\bigg\langle#2\bigg\rangle}%
{4}{\Bigg\langle#2\Bigg\rangle}%
}[\PackageError{inner}{Undefined option to inner: #1}{}]%
}
\newcommand{\abs}[2][a]{
\IfEqCase{#1}{%
{a}{\left\vert#2\right\rvert}%
{0}{\vert#2\rvert}%
{1}{\big\vert#2\big\rvert}%
{2}{\Big\vert#2\Big\rvert}%
{3}{\bigg\vert#2\bigg\rvert}%
{4}{\Bigg\vert#2\Bigg\rvert}%
}[\PackageError{inner}{Undefined option to abs: #1}{}]%
}



%\newcommand{\set}[1]{\left\{#1\right\}}


% Autres

\newcommand{\np}{_{_-}}
\newcommand{\pp}{_{_+}}
\newcommand{\defeq}{\stackrel{\cdot}{=}} % this is for
                                % definition-equal, not for number 2
                                % [This comment is (c) Gabór L. ]
\newcommand{\bydef}{:=}       % an alternative to defeq

% Operateurs proba

%\newcommand{\var}[2][a]{{\rm Var}\brac[#1]{#2}}
\newcommand{\cov}[2][a]{{\rm Cov}\brac[#1]{#2}} 
%\newcommand{\e}[2][a]{\mbe\brac[#1]{#2}}
\newcommand{\ee}[3][a]{\mbe_{#2}\brac[#1]{#3}}
\newcommand{\prob}[2][a]{\mbp\brac[#1]{#2}}
\newcommand{\probb}[3][a]{\mbp_{#2}\brac[#1]{#3}}


% Operateurs

\def\argmin{\mathop{\rm arg\,min}\limits}
\def\argmax{\mathop{\rm arg\,max}\limits}
\def\sgn{\mathop{\rm Sgn}\limits}
\def\tr{\mathop{\rm Tr}\limits}
\def\rank{\mathop{\rm rank}}

% abbrev lettres grecques

\newcommand{\al}{\alpha}
\newcommand{\lam}{\lambda}
\newcommand{\om}{\omega}
\newcommand{\eps}{\varepsilon}

% abbrev lettres mathcal

\def\cA{{\mtc{A}}}
\def\cB{{\mtc{B}}}
\def\cC{{\mtc{C}}}
\def\cD{{\mtc{D}}}
\def\cE{{\mtc{E}}}
\def\cF{{\mtc{F}}}
\def\cG{{\mtc{G}}}
\def\cH{{\mtc{H}}}
\def\cI{{\mtc{I}}}
\def\cK{{\mtc{K}}}
\def\cL{{\mtc{L}}}
\def\cM{{\mtc{M}}}
\def\cN{{\mtc{N}}}
\def\cO{{\mtc{O}}}
\def\cP{{\mtc{P}}}
\def\cQ{{\mtc{Q}}}
\def\cR{{\mtc{R}}}
\def\cS{{\mtc{S}}}
\def\cT{{\mtc{T}}}
\def\cU{{\mtc{U}}}
\def\cV{{\mtc{V}}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}

% abbrev lettres mathbb

\newcommand{\mbe}{\mathbb{E}}
\newcommand{\mbr}{\mathbb{R}}
\newcommand{\mbp}{\mathbb{P}}
\newcommand{\mbq}{\mathbb{Q}}
\newcommand{\mbi}{\mathbb{I}}
\newcommand{\mbn}{\mathbb{N}}
\newcommand{\mbz}{\mathbb{Z}}
\newcommand{\mbs}{\mathbb{S}}
\newcommand{\mbk}{\mathbb{K}}
\newcommand{\mbg}{\mathbb{G}}
\newcommand{\mbv}{\mathbb{V}}


% abbrev lettres en gras

\newcommand{\bA}{{\mbf{A}}}
\newcommand{\bB}{{\mbf{B}}}
\newcommand{\bD}{{\mbf{D}}}
\newcommand{\bG}{{\mbf{G}}}
\newcommand{\bI}{{\mbf{I}}}
\newcommand{\bJ}{{\mbf{J}}}
\newcommand{\bW}{{\mbf{W}}}
\newcommand{\bX}{{\mbf{X}}}
\newcommand{\bY}{{\mbf{Y}}}
\newcommand{\bZ}{{\mbf{Z}}}


\newcommand{\bp}{{\mbf{p}}}
\newcommand{\boldf}{{\mbf{f}}}
\newcommand{\bx}{{\mbf{x}}}
\newcommand{\by}{{\mbf{y}}}
\newcommand{\bz}{{\mbf{z}}}
\newcommand{\bw}{{\mbf{w}}}
\newcommand{\bv}{{\mbf{v}}}
\newcommand{\barx}{{\bar{x}}}
\newcommand{\beps}{{\mbf{\varepsilon}}}


% frak

\newcommand{\fP}{{\mathfrak{P}}}
\newcommand{\fK}{{\mathfrak{K}}}



% TODO command

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% A command to put notes in a draft

%\newcounter{nbdrafts}
%\setcounter{nbdrafts}{0}
%\makeatletter
%\newcommand{\checknbdrafts}{
%\ifnum \thenbdrafts > 0
%\@latex@warning@no@line{**********************************************************************}
%\@latex@warning@no@line{* The document contains \thenbdrafts \space draft note(s)}
%\@latex@warning@no@line{**********************************************************************}
%\fi}
%\newcommand{\todo}[1]{\addtocounter{nbdrafts}{1}{\color{awesome} #1}}
%\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcounter{nbnotes}
\setcounter{nbnotes}{0}
\makeatletter
\newcommand{\checknbnotes}{
\ifnum \thenbnotes > 0
\@latex@warning@no@line{**********************************************************************}
\@latex@warning@no@line{* The document contains \thenbnotes \space color note(s)}
\@latex@warning@no@line{**********************************************************************}
\fi}
\newcommand{\note}[1]{\addtocounter{nbnotes}{1}{\color{blue} #1}}%amethyst
\makeatother

